MSP: An FPGA-Specific Mixed-Scheme, Multi-Precision Deep Neural Network Quantization Framework

With the tremendous success of deep learning, there exists imminent need to deploy deep learning models onto edge devices. To tackle the limited computing and storage resources in edge devices, model compression techniques have been widely used to trim deep neural network (DNN) models for on-device inference execution. This paper targets the commonly used FPGA (field programmable gate array) devices as the hardware platforms for DNN edge computing. We focus on the DNN quantization as the main model compression technique, since DNN quantization has been of great importance for the implementations of DNN models on the hardware platforms. The novelty of this work comes in twofold: (i) We propose a mixed-scheme DNN quantization method that incorporates both the linear and non-linear number systems for quantization, with the aim to boost the utilization of the heterogeneous computing resources, i.e., LUTs (look up tables) and DSPs (digital signal processors) on an FPGA. Note that all the existing (single-scheme) quantization methods can only utilize one type of resources (either LUTs or DSPs for the MAC (multiply-accumulate) operations in deep learning computations. (ii) We use a quantization method that supports multiple precisions along the intra-layer dimension, while the existing quantization methods apply multi-precision quantization along the inter-layer dimension. The intra-layer multi-precision method can uniform the hardware configurations for different layers to reduce computation overhead and at the same time preserve the model accuracy as the inter-layer approach.

==> Section/5_results_bk.tex <==
\section{Evaluation}\label{sec:eva}

\subsection{Experiment Setup}

\begin{table*}[ht]
\small
\centering
\tabcolsep 8pt
\renewcommand\arraystretch{1.1}
\begin{tabular}{c c c c c c}%{p{0.25\linewidth}p{0.25\linewidth}p{0.25\linewidth}p{0.25\linewidth}}
\toprule
Quantization & Bit width & \multicolumn{2}{c}{ResNet-18 Accuracy (\%)} & \multicolumn{2}{c}{MobileNet-v2 Accuracy (\%)} \\
Scheme & (Wght./Actv.) & Top1 (N/Y) & Top5 (N/Y)& Top1 (N/Y) & Top5 (N/Y)\\
\hline
\multicolumn{6}{c}{\textbf{CIFAR-10}} \\
\hline
Baseline  & 32/32 & 93.62 & - & 92.51 & -\\
PoT & 4/4 &92.97
/ 92.14& - & 91.34 / 90.92&-\\
Fixed & 4/4 & 93.43 / 92.97 & - & 92.34 / 91.76 & -\\
SPoT & 4/4 & 93.47
/ 92.94 & - & 92.72
/ 91.83& -\\
MS& 4/4 & 93.53
/ 92.98& - & 92.57
/ 91.99& -\\
MP & 4/4 & - / 93.63
&-  & - / 92.54
&- \\
\bf{MSP} & 4/4 & - / \bf{93.72}
&-  & - / \bf{92.58}
&- \\
\hline
\multicolumn{6}{c}{\textbf{CIFAR-100}} \\
\hline
Baseline & 32/32 &  74.49&  92.70& 71.48& 91.98\\
PoT & 4/4 &73.88
/ 72.97 &92.14
/ 91.65 &68.68
/ 67.11& 90.06
/ 89.21\\
Fixed & 4/4 &  74.37
/ 73.88&  92.31 / 91.72& 71.16
/ 70.22 & 91.63
/ 90.88\\
SPoT & 4/4 &  74.33
/ 73.97&  92.49
/ 92.03 & 71.13
/ 70.21& 91.69
/ 90.85\\
MS & 4/4 & 74.58
/ 74.03& 92.51
/ 92.05 & 71.21
/ 70.25& 91.74
/ 90.92 \\
MP & 4/4 & - / 74.54
& - / 92.61
& - / 71.49
& - / 91.82 \\
\bf{MSP} & 4/4 & - / \bf{74.61}
& - / \bf{92.69}
& - / \bf{71.51}
& - / \bf{91.97} \\
\hline
 & &\multicolumn{2}{c}{\textbf{ImageNet}} & \multicolumn{2}{c}{Wght./Actv. 4/32} \\
\hline
Baseline & 32/32 & 69.76 & 89.08 & 71.88& 90.29\\
PoT &4/4 &68.20
/ 67.11 &87.14
/ 85.93& 69.93 / 67.88& 88.63 / 86.83\\
Fixed & 4/4 & 69.72
/ 68.66 &  88.67
/ 87.54& 71.26
/ 69.23& 90.18 / 88.03 \\
SPoT& 4/4 & 69.74
/ 68.48 &  88.71
/ 87.92 & 71.32
/ 69.76& 90.17
/88.42\\
MS & 4/4 &  70.11
/ 69.22 & 89.41
/ 88.33& 71.26
/ 69.31& 90.04
/ 88.11\\
MP & 4/4 & - / 69.99 
& - / 89.12 
& - / 71.68 & - / 90.22\\
\bf{MSP} & 4/4 & - / \bf{70.47} 
& - / \bf{89.52} 
& - / \bf{71.73} & - / \bf{90.27}\\

\bottomrule
\end{tabular}
\caption{Result from different quantization schemes for the ResNet-18 and MobileNet-v2 DNN models on CIFAR-10, CIFAR-100, and ImageNet datasets. Y/N: With/Without quantization of the first and the last layer.}
\label{tab:comparison_schemes}
\end{table*}

\begin{table}[t]
\small
\centering
\tabcolsep 2.2pt
% \renewcommand\arraystretch{1.1}
\begin{tabular}{ccccc}%{p{0.25\linewidth}p{0.25\linewidth}p{0.25\linewidth}p{0.25\linewidth}}
\toprule
\multirow{2}{*}{Methods} & Top-1 & Top-5 &
quant. &
quant.\\
~  & (\%) & (\%) &1st $l$.& Last $l$.\\
\hline
Baseline  & 69.76 & 89.08& -& -\\
Dorefa ~\cite{zhou2016dorefa}  & 68.10 & 88.10&$\times$&$\times$\\
PACT ~\cite{choi2018pact} & 69.20 & 89.00&$\times$&$\times$\\
DSQ ~\cite{gong2019differentiable}  & 69.56 & N/A&$\times$&$\times$\\
%LSQ\cite{esser2019learned} & 4/4 & 71.10 & 90.00\\
QIL ~\cite{jung2019learning}  & 70.10 & N/A&$\times$&$\times$\\
%APoT\cite{li2019additive} & 4/4 & 70.70 & 89.60\\
$\mu$L2Q ~\cite{cheng2019uL2Q}  & 65.92 & 86.72&-&16bit\\
LQ-NETS ~\cite{zhang2018lq} & 69.30 & 88.80&$\times$&$\times$\\
\textbf{MSP (ours)}  & \textbf{70.47} & \textbf{89.52}&\textbf{\checkmark}&\textbf{\checkmark}\\

\bottomrule
\end{tabular}
\caption{Comparisons with existing works with ResNet-18 model on ImageNet dataset for 4 bit quantization.} \label{tab:imagenetresnet}
\end{table}

\begin{table}[htb]
% \setlength\tabcolsep{5pt}
\small
\centering
\begin{tabular}{c|c|cccc|cc}
    \toprule
    \multirow{3}{*}{Device} & \multirow{3}{*}{\makecell{Ratio \\ (SPoT/4-bit/8-bit)}} & \multicolumn{4}{c|}{Utilization} & \multicolumn{2}{c}{Throughput (GOPS)} \\
    \cline{3-8}
    ~ & ~ & \multirow{2}{*}{LUT} & \multirow{2}{*}{DSP} & \multirow{2}{*}{BRAM36} & \multirow{2}{*}{FF} & ResNet-18 & MobileNet-v2  \\
    ~ & ~ & ~ & ~ & ~ & ~ & on ImageNet & on ImageNet \\
    \hline
    \multirow{4}{*}{XC7Z020} & 0:1:0 & 12.2K (23\%) & 220 (100\%) & 39 (56\%) & 9.4K (9\%) & 31.8 & 26.6 \\
    ~ & 1:1:0 & 22.9K (43\%) & 220 (100\%) & 49 (70\%) & 14.5K (14\%) & 51.6 & 47.4 \\
    ~ & 1.5:1:0 & 28.3K (53\%) & 220 (100\%) & 56 (80\%) & 17.1K (16\%) & 58.2 & 55.3 \\
    ~ & 60:35:5 (MSP) & 31.1K (58\%) & 220 (100\%) & 59 (84\%) & 20.5K (19\%) & \textbf{73.8} & \textbf{58.7} \\
    \hline
    \multirow{4}{*}{XC7Z045} & 0:1:0 & 41.8K (19\%) & 900 (100\%) & 160 (29\%) & 31.3K (7\%) & 120.5 & 102.8 \\
    ~ & 1:1:0 & 93.4K (43\%) & 900 (100\%) & 194 (36\%) & 65.7K (15\%) & 195.3 & 190.6 \\
    ~ & 2:1:0 & 145.0K (66\%) & 900 (100\%) & 225.5 (41\%) & 111.6K (26\%) & 244.5 & 236.5 \\
    ~ & 65:30:5 (MSP) & 151.4K (69\%) & 900 (100\%) & 245 (45\%) & 114.2K (26\%) & \textbf{325.0} & \textbf{262.2} \\
    \bottomrule
\end{tabular}
\caption{Performance of various DNN applications on hardware under different settings.}
\label{tab:perf}
\end{table}

\begin{table}[t]
\small
\centering
\tabcolsep 3pt
\renewcommand\arraystretch{1.1}
\begin{tabular}{ccccccccccccccccc}
\toprule
 &  & \textbf{MSP} & MSP & MSP & MP & MS & MS & MS &Fixed & Fixed & PoT & PoT & SPoT & SPoT \\
 \hline
\multirow{2}{*}{DSP} & 8-bit FP & 5\% & 5\% & 10\% & 5\% & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 & 4-bit FP & 30\% & 0 & 0 & 95\% & 50\% & 50\% & 33\% & 100\% & 100\% & 0 & 0 & 0 & 0 \\
\multirow{2}{*}{LUT} & 4-bit SPoT & 65\% & 95\% & 90\% & 0 & 50\% & 50\% & 67\% & 0 & 0 & 0 & 0 & 100\% & 100\% \\
 & 4-bit PoT & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 100\% & 100\% & 0 & 0 \\
\multicolumn{2}{c}{First and Last Layer (Y/N)} & Y & Y & Y & Y & N & Y & N & N & Y & N & Y & N & Y \\
\hline
\multicolumn{2}{c}{Top-1 Accuracy (\%)} & \textbf{70.47} & 70.09 & 70.24 & 69.99 & 70.08 & 69.52 & 70.11 & 69.72 & 68.66 & 68.20 & 67.11 & 69.74 & 68.48 \\
\multicolumn{2}{c}{FPGA Latency (ms)} & \bf{11.2} & 13.7 & 13.3 & 29.1 & 20.1 & 12.2 & 15.4 & 39.5 & 25.4 & 19.5 & 14.7 & 22.9 & 16.5 \\
\bottomrule
\end{tabular}
\caption{Ablation study of ResNet-18 on ImageNet. Y/N: With/Without quantization of the first and the last layer. The results are measured on XC7Z045.}
\label{tab:ablation}
\end{table}

We evaluate our novel MSP on image classification tasks with convolutional neural networks (CNNs). We use no extra data augmentations other than those already employed for training the 32-bit floating-point baseline models. Our quantization training algorithm uses step or cosine learning rate decay and $\ell_2$ regularization, following training algorithms of the baseline models. Our experiments are implemented with server-grade machines running Ubuntu 18.04, CUDA
10.2 and PyTorch 1.5. Our models are trained on NVIDIA TITAN RTX GPUs and GeForce RTX 2080Ti GPUs.
We evaluate with the deep residual net (ResNet-18)~\cite{he2016deep}, which generalizes well for varieties of tasks, as well as the lightweight MobileNet-v2 model ~\cite{sandler2018mobilenetv2}.
We test on CIFAR-10, CIFAR-100 ~\cite{krizhevsky2009learning}, and ImageNet ILSVRC-2012 ~\cite{krizhevsky2012imagenet} datasets.
DNN models for CIFAR-10 and CIFAR-100 datasets are trained from scratch, and quantized for $150$ epochs.
For ImageNet dataset, pre-trained models in 32-bit floating-point are used, and quantized for $90$ epochs. 
The initial learning rates are $8e-3$ for CIFAR-10, $4e-3$ for CIFAR-100, $1e-2$ for ImageNet.

To demonstrate hardware efficiency of the proposed MSP framework, we implemented the architecture with heterogeneous $GEMM$ cores on the embedded FPGA device, in which high efficiency is usually top priority under resource constraints. We validate our framework on Zynq XC7Z020 and XC7Z045 devices with different design parameters that result in different throughput and resource utilization results.
We setup different ratios between the PE array sizes of the $GEMM_{SPoT}$,$GEMM_{fixed}$, and $GEMM_{8-bit}$ cores. 
Specifically, we progressively increase the size of $GEMM_{SPoT}$ core ($Blk_{out,SPoT}$), till the LUT utilization reaches the highest ratio.
For all implementations, the working frequency is set to 100MHz.


\subsection{Accuracy Performance}
%\yanyu{We evaluate our novel intra-layer mixed scheme quantization on image classification tasks. Comparing to 8+4+8, our method achieve comparable or even higher accuracy with first and last layer quantized to low bit width as well. }

Tables \ref{tab:comparison_schemes} and \ref{tab:imagenetresnet} summarize quantization results for image classification task.
% Table \ref{tab:comparison_schemes} compares different quantization schemes including power-of-2 (P2), fixed-point (Fixed), sum-of-power-of-2 (SPoT), mixed-scheme quantization (MS), multi-precision quantization (MP), and our MSP quantization scheme. 
We use $PR_{SPoT:Fixed:8-bit}=65:30:5$, which is the optimal ratio validated from resource utilization results on FPGA. MSP obtains the minimum accuracy degradation.

The accuracy increase of MSP compared to PoT, Fixed, SPoT, MS or MP results from several aspects. First, combining SPoT and Fixed makes the quantized DNN weights fit the original weight distribution better. Besides, leave $5\%$ weight with 8-$bit$, which is "intra-layer flexibility" can achieve lossless performance even the first and the last layer are quantized.
In addition, model compression could slightly increase accuracy when weight bit-width $\geq 4$, as 
% the quantization resolution is high enough so that the inference results of DNNs are not affected, and 
quantization noise can potentially act as regularization that benefits generalization and addresses overfitting.

%We also provide a comparison between whether quantize the first and the last layer. Table \ref{tab:comparison_schemes} shows that when we quantize the first and the last layer, the accuracy  decreases $1\%$ on the ImageNet of ResNet-18. Even on CIFAR-10 and CIFAR-100 datasets, quantize the first and the last layer still causes $0.5\%$ accuracy degradation. For the MobileNet-v2, accuracy degradation is more obvious (e.g. $2\%$ on the ImageNet and $1\%$ on CIFAR-10 and CIFAR-100). Since the first and the last layer are more sensitive, that is why the other existing works do not quantize the first and the last layer. 
Tables \ref{tab:imagenetresnet}  compares our MSP with existing DNN quantization works including Dorefa ~\cite{zhou2016dorefa},
PACT ~\cite{choi2018pact},
DSQ ~\cite{gong2019differentiable},
QIL ~\cite{jung2019learning},
$\mu$L2Q ~\cite{cheng2019uL2Q}, and
LQ-NETS ~\cite{zhang2018lq}.
Those works and our MSP start with the same pre-trained models with the same baseline accuracy.
Table \ref{tab:imagenetresnet} shows that Dorefa, PACT, DSQ, $\mu$L$2$Q, and LQ-NETS have up to $3.84\%$ accuracy degradation, only QIL reports lossless accuracy performance. Our MSP increases accuracy by $0.71\%$ compared with the floating-point model. Note that those works above they do not quantize the first and the last layer, only $\mu$L2Q uses 16bit weight representation for the last layer. On the other hand, MSP quantizes the first and the last layer while still can achieve the lossless accuracy performance.

\subsection{Hardware Efficiency}
%\yanyu{Latency, comparison with 8+4+8. }

To present the performance with real-world applications, we employed different CNN models with the proper SPoT/fixed-point/8-bit ratios on the two devices. The networks ResNet-18 and MobileNet-v2 are implemented based on the ImageNet dataset. The performance results of each network under various hardware configurations are displayed in Table \ref{tab:perf}. 
%Generally, the overall PE utilization reaches $38.75\%$ to $72.5\%$,
Generally, the utilization of DSP is always $100\%$, by increasing the ratio of SPoT, the utilization of the other resource has improved (e.g. from $19\%$ to $69\%$ on LUT in XC7Z045).
On the other hand, the heterogeneous $GEMM_{SPoT}$, $GEMM_{fixed}$, and $GEMM_{8-bit}$ cores improve the throughput by $2.2\times-2.7\times$ with the optimal design compared to utilizing the $GEMM_{fixed}$ core only
(e.g. the throughput from 120.5 to 325.0 GOPS on ResNet-18 in XC7Z045). %MobileNet-v2 has the most complicated structure among all these networks, making it difficult to deploy on hardware platforms, but our designs can still achieve high performance.

\subsection{Ablation Study}
We experiment over different quantization configurations to validate the proposed MSP scheme. Note that all the percentages refer to the ratio of employed quantization scheme in the main body of a DNN, since first and last layers are specified separately. As shown in table \ref{tab:ablation}, single scheme quantization (fixed point ~\cite{zhou2016dorefa}, PoT, SPoT) shows no advantage in both accuracy and speed (FPGA latency in our work). Plus, simply quantizing first and last layer into low bit width introduces noticeable accuracy degradation. With our Mixed Scheme (MS) method, execution speed is increased significantly because of efficient utilization of both DSP and LUTs. We can also observe slight improvement in accuracy, because the dual schemes are organized to better fit weight distribution, as described in \ref{sec:sp2}. Finally we employ our intra-layer mixed precision (MP) to mitigate the need of high bit widths in first and last layers, further improving speed and achieving comparable accuracy. 

